Revisit Large-Scale Image-Caption Data in Pre-training Multimodal Foundation Models

Recent advancements in multimodal models highlight the value of rewritten captions for improving performance, yet key challenges remain. For example, while synthetic captions often provide superior quality and image-text alignment, it is not clear whether they can fully replace AltTexts: the role of synthetic captions and their interaction with original web-crawled AltTexts in pre-training is still not well understood. Moreover, different multimodal foundation models may have unique preferences for specific caption formats, but efforts to identify the optimal captions for each model remain limited. In this work, we propose a novel, controllable, and scalable captioning pipeline designed to generate diverse caption formats tailored to various multimodal models. By examining Short Synthetic Captions (SSC) towards Dense Synthetic Captions (DSC+) as case studies, we systematically explore their effects and interactions with AltTexts across models such as CLIP, multimodal LLMs, and diffusion models. Our findings reveal that a hybrid approach that keeps both synthetic captions and AltTexts can outperform the use of synthetic captions alone, improving both alignment and performance, with each model demonstrating preferences for particular caption formats. This comprehensive analysis provides valuable insights into optimizing captioning strategies, thereby advancing the pre-training of multimodal foundation models.

==> Notes.tex <==
https://arxiv.org/pdf/2306.07952.pdf

https://arxiv.org/pdf/2307.10350.pdf

https://arxiv.org/pdf/2305.20088.pdf



==> Table/clip_v2.tex <==

\begin{table}[t]
\begin{tabular}{c}

\hspace{-0.15cm}%
\begin{minipage}[t]{0.8\linewidth}
\vspace{0pt}
\centering


\caption{\small{Effect of different synthetic captions on CLIP with ViT-B/16 as the backbone.
}}
\vspace{-0.2cm}
\label{tab:vecap_clip}   
\small
\resizebox{1.0\textwidth}{!}{
  \begin{tabular}{ccccc|ccc}
        \toprule[1.2pt]
        \multirow{2}{*}{\bf Pre-train Caption}  & \multicolumn{2}{c}{\bf COCO (R@1)} & \multicolumn{2}{c}{\bf Flickr30k (R@1)} & \multirow{2}{*}{\bf ImageNet} & \multirow{2}{*}{\bf Linear Probing} & \multirow{2}{*}{\bf ImageNetV2}  \\
         & \bf I-T & \bf T-I & \bf I-T & \bf T-I & & & \\
        \midrule
        AltText  & 54.24 & 36.98 & 81.30 & 65.80 & 65.70 & 58.58 \\
        % AltText & AltText & 53.72 & 36.89 & \textbf{81.90} & 65.72 & 65.62 & 58.39 \\
        % \midrule
        DSC  & 52.28 & 29.00 & 80.90 & 54.75 & 27.30 & 21.91 \\
        % DSC + AltText & - &65.84	&46.08	&90.26	&73.94	&66.18	&58.74 \\
        % DSC & AltText & \textbf{64.10} & \textbf{41.47} & \textbf{90.20} & \textbf{68.14} & \textbf{49.26} & \textbf{42.61} \\
        % \midrule
        SSC & 57.00 & 35.15 & 84.67 & 63.35 & 49.10 & 43.31 \\
        % SSC & AltText & \textbf{58.18} & \textbf{42.03} & \textbf{88.10} & \textbf{70.10} & \textbf{58.90} & \textbf{52.01} \\
        % \midrule
        DSC + AltText  &65.84	&46.08	&90.26	&73.94	&66.18	&58.74 \\
        SSC + AltText  & 66.67	&48.13	&91.81	&76.54	&\textbf{66.63}	& \textbf{59.57} \\
        DSC + SSC + AltText  & \textbf{69.88}	& \textbf{50.28}	& \textbf{93.50}	& \textbf{77.19} &	65.16	& 58.11 \\
        % DSC + SSC + AltText & AltText & \textbf{70.08} & \textbf{50.59} & 93.11 &\textbf{77.78} &\textbf{66.39}	& \textbf{59.53} \\

        \bottomrule[1.2pt]
    \end{tabular}
}



\end{minipage}

% &
% \hspace{-0.3cm}%
% \begin{minipage}[t]{0.40\linewidth}
% \vspace{0pt}


% \includegraphics[width=\linewidth]{Figure/lp.png}
% \vspace{-0.8cm}
% % \captionof{figure}{\footnotesize{Evaluation with linear probing.}}
% \captionof{figure}{\footnotesize Evaluation with linear probing.}
% \label{fig:linear_probing}


% \end{minipage}


\end{tabular}
\vspace{-0.2cm}
\end{table}


